Asynchronous Communication: Capacity Bounds and Suboptimality of Training

Several aspects of the problem of asynchronous point-to-point communication without feedback are developed when the source is highly intermittent. In the system model of interest, the codeword is transmitted at a random time within a prescribed window whose length corresponds to the level of asynchronism between the transmitter and the receiver. The decoder operates sequentially and communication rate is defined as the ratio between the message size and the elapsed time between when transmission commences and when the decoder makes a decision. For such systems, general upper and lower bounds on capacity as a function of the level of asynchronism are established, and are shown to coincide in some nontrivial cases. From these bounds, several properties of this asynchronous capacity are derived. In addition, the performance of training-based schemes is investigated. It is shown that such schemes, which implement synchronization and information transmission on separate degrees of freedom in the encoding, cannot achieve the asynchronous capacity in general, and that the penalty is particularly significant in the high-rate regime.

==> NOTES <==
* \nu vs n distinction not so important.  same issue arises for m

* fig 3 axis should be replaced with R/C instead of R

* can't use \cD_N in rate def...caligraphic fonts for sets/events

* replace example of Fig. 5 with Z channel.   simpler.

* add missing 0 to output node of example of fig. 4

* fix training based section to eliminate having two definitions, as
  we discussed.

==> NOTES-gww <==
bibiog out of date; also add to bibiog:

@InProceedings{WCCW,
  author = 	 {D. Wang and V. Chandar and  S.-Y. Chung and G. W. Wornell},
  title = 	 {Error Exponents in Asynchronous Communication},
  booktitle =	 {Proc.\ Int.\ Symp.\ Inform.\ Theory},
  year =	 {2011},
  address =	 {St.\ Petersburg, Russia},
  month =	 {July}
}

also, had to remove amsthm -- IEEE will eliminate

adjusted \defeq

considered of self-interest = of independent interest
also, why important?

Section IV-A, paragraph 2:  three error types   

Section IV-A, paragraph 3.  vague

Section IV-A, paragraph 4:  "the error probability"...overall?

after eq (5):   aren't most LB tight?

Thm 3:  why don't we let sigma_0=1 wolg?   and then replace p with
\rho

eq (7):   label RHS alpha_UB(R) or \bar{alpha}(R)

Fig. 4:   label outputs with 0 and 1, and put *=0 at input?

Fig. 6:  lines too thin and fonts too small

Figs 6 and 7 and 10:   normalize horizontal axis so R/C

can't end examples with QED symbol

footnote 9:  why are units of distance?

Example 1 split into two: 1 and 2

Examples 1 and 2:   asymmetric/symmetric noise ambiguous.  modulo 2
noise in channel when codeword present is symmetric always.

Example 4 (now 5) of Fig 10, third paragraph:  important?

Fig. 11:  label top curve:  TUB, UB

Remark 2  before Section V-B:   why do we care about this
strengthening (and App A)?

V-B first paragraph:  FIXME...






==> NOTES-gww_ <==
bibiog out of date

also add to bibiog:


@InProceedings{WCCW,
  author = 	 {D. Wang and V. Chandar and  S.-Y. Chung and G. W. Wornell},
  title = 	 {Error Exponents in Asynchronous Communication},
  booktitle =	 {Proc.\ Int.\ Symp.\ Inform.\ Theory},
  year =	 {2011},
  address =	 {St.\ Petersburg, Russia},
  month =	 {July}
}




==> NOTES_ <==
\nu vs n distinction not so important.  same issue arises for m


==> abstract.tex <==
Several aspects of the problem of asynchronous point-to-point
communication without feedback are developed when the source is highly
intermittent.  In the system model of interest, the codeword is
transmitted at a random time within a prescribed window whose length
corresponds to the level of asynchronism between the transmitter and
the receiver. The decoder operates sequentially and communication rate
is defined as the ratio between the message size and the elapsed time
between when transmission commences and when the decoder makes a
decision.

For such systems, general upper and lower bounds on capacity as a
function of the level of asynchronism are established, and are shown
to coincide in some nontrivial cases.  From these bounds, several
properties of this asynchronous capacity are derived.  In addition,
the performance of training-based schemes is investigated. It is shown
that such schemes, which implement synchronization and information
transmission on separate degrees of freedom in the encoding, cannot
achieve the asynchronous capacity in general, and that the penalty is
particularly significant in the high-rate regime.


==> binsym.tex <==
\setlength{\unitlength}{0.8bp}%
\begin{picture}(0,0)
\includegraphics[scale=0.8]{binsym}
\end{picture}%
\begin{picture}(92,74)


\put(-8,0){\makebox(0,0){$1$}}
\put(-8,73){\makebox(0,0){$\star$}}



\end{picture}
\vspace{0.5cm}


==> binsymno.tex <==
\setlength{\unitlength}{0.8bp}%
\begin{picture}(0,0)
\includegraphics[scale=0.8]{binsymno}
\end{picture}%
\begin{picture}(92,146)

\put(-8,146){\makebox(0,0){$\star$}}
\put(60,110){\makebox(0,0){\footnotesize{$1/2$}}}
\put(15,100){\makebox(0,0){\footnotesize{$1/2$}}}

\put(-8,0){\makebox(0,0){$1$}}
\put(-8,73){\makebox(0,0){$0$}}



\end{picture}
\vspace{0.5cm}


==> channelmodel2.tex <==
\setlength{\unitlength}{0.8bp}%
\begin{picture}(0,0)
\includegraphics[scale=0.8]{channelmodel2}
\end{picture}%
\begin{picture}(74, 146)

\put(-15,89){\makebox(0,0){$\cal{X}$}}

\put(90,89){\makebox(0,0){$\cal{Y}$}}
\put(-6,31){\makebox(0,0){$\star$}}

\put(37,166){\makebox(0,0){$W(\cdot|\cdot)$}}




\end{picture}
\vspace{0.5cm}


==> distin.tex <==
\setlength{\unitlength}{0.8bp}%
\begin{picture}(0,0)
\includegraphics[scale=0.8]{distin}
\end{picture}%
\begin{picture}(92,74)


\put(-8,0){\makebox(0,0){$1$}}
\put(-8,73){\makebox(0,0){$\star$}}



\end{picture}
\vspace{0.5cm}


==> zno.tex <==
\setlength{\unitlength}{0.8bp}%
\begin{picture}(0,0)
\includegraphics[scale=0.8]{zno}
\end{picture}%
\begin{picture}(92,146)


\put(-8,146){\makebox(0,0){$\star$}}
\put(-8,0){\makebox(0,0){$1$}}
\put(-8,73){\makebox(0,0){$0$}}
\put(60,110){\makebox(0,0){\footnotesize{$1/2$}}}
\put(15,100){\makebox(0,0){\footnotesize{$1/2$}}}




\end{picture}
\vspace{0.5cm}

